Legal Case Document Similarity: You Need Both Network and Text

Estimating the similarity between two legal case documents is an important and challenging problem, having various downstream applications such as prior-case retrieval and citation recommendation. There are two broad approaches for the task -- citation network-based and text-based. Prior citation network-based approaches consider citations only to prior-cases (also called precedents) (PCNet). This approach misses important signals inherent in Statutes (written laws of a jurisdiction). In this work, we propose Hier-SPCNet that augments PCNet with a heterogeneous network of Statutes. We incorporate domain knowledge for legal document similarity into Hier-SPCNet, thereby obtaining state-of-the-art results for network-based legal document similarity. Both textual and network similarity provide important signals for legal case similarity; but till now, only trivial attempts have been made to unify the two signals. In this work, we apply several methods for combining textual and network information for estimating legal case similarity. We perform extensive experiments over legal case documents from the Indian judiciary, where the gold standard similarity between document-pairs is judged by law experts from two reputed Law institutes in India. Our experiments establish that our proposed network-based methods significantly improve the correlation with domain experts' opinion when compared to the existing methods for network-based legal document similarity. Our best-performing combination method (that combines network-based and text-based similarity) improves the correlation with domain experts' opinion by 11.8% over the best text-based method and 20.6\% over the best network-based method. We also establish that our best-performing method can be used to recommend / retrieve citable and similar cases for a source (query) case, which are well appreciated by legal experts.

==> sections/eval-second.tex <==


Recall from Section~\ref{sec:dataset} that the evaluation dataset used in this work contains an almost equal number of similar document-pairs and dissimilar document-pairs. 
Till now, we have been giving equal weightage to both the `similar' and `dissimilar' document-pairs while evaluating the methods.
But in practice, the chance that two randomly selected legal documents will be similar is much lower; 
hence, the `similar' class is the minority class in our setting.
%Therefore, it is much easier to label a document-pair as `dissimilar' than `similar'. It is a niche task especially in Legal IR to correctly identify a much smaller set of similar documents. 
Also, it is a more risky/serious error to label a document-pair that is actually `similar' as `dissimilar' (since a Law practitioner may miss a very relevant prior case), than labelling an actually `dissimilar' document-pair as `similar'. 

We therefore introduce weighted metrics for evaluation in this section. The idea is to \textit{reward a method more for correctly labeling similar document-pairs}, than for labeling dissimilar document-pairs correctly, because the later is relatively much easier. 
In a classification setup in our context, methods that identify true positives (similar document-pairs) correctly are better than methods identifying true negatives (dissimilar document-pairs) correctly.  

We first define the weighted evaluation metrics we use, and then discuss how we decide the weights for the similar document-pairs and the dissimilar document-pairs.


\new{\subsection{Weighted evaluation metrics}}

In the weighted metrics, we assign a weight $w_1$ to the `similar' class and a different weight $w_0$ to the `dissimilar' class ($w_1 > w_0$); we will define later how we decide the values $w_0$ and $w_1$. 
For now, we apply the weighting mechanism to the evaluation metrics FScore and MSE. 
Redesigning Pearson Correlation Coefficient by incorporating weights is a scope of future work. 
The weighted FScore and MSE metrics are defined as follows:

\vspace{2mm}
\noindent \textbf{(i) Wtd. Fscore} is calculated by weighing the FScores of the `similar' class and the `dissimilar' class:
\begin{equation}
\mbox{Wtd. FScore} = \frac{(w_0 * F_0) + (w_1 * F_1)}{w_0 + w_1}
\end{equation}
where $F_0$ and $F_1$ are the FScore of the `dissimilar' and `similar' class respectively.

\vspace{2mm}
\noindent \textbf{(ii) Wtd. MSE}: In this metric, we weigh the Mean Squared Error between the expert scores and the algorithmic scores. For a particular document-pair $i$, we have two similarity scores: $y_i \in [0,1]$ which is the expert-assigned similarity score and $\hat{y}_i \in [0,1]$ given by a method. 
If $y_i > 0.5$, we consider the document-pair $i$ to be `similar' and assign the weight to document pair $i$ as $w_i = w_1$ , else $w_i = w_0$. 
The weighted squared error for the document-pair $i$ is $w_i * (y_i - y_i)^2$. This implies that for a similar document-pair, the difference between the expert-assigned score and the method-generated score is penalized more than that for a dissimilar document-pair. 
The wtd. Mean Square Error, across all document-pairs, is calculated as
\begin{equation}
\mbox{Wtd. MSE} = \frac{\sum_{i=1}^{n} w_i * (y_i - \hat{y_i})^2}{\sum_{i=1}^{n}w_i} 
\end{equation}


\new{\subsection{Deciding the weights}}

We now describe two different approaches by which we decide the weights $w_0$ and $w_1$ for the `dissimilar' and `similar' classes respectively. The basic hypothesis is that since the probability of the `similar' class is much lower than that of the `dissimilar' class, a similar document-pair should be assigned a much higher weight than a dissimilar document-pair. 
In other words, the weight of a particular class is the inverse of its probability. 
Hence, the weight of the `similar' class $w_1 = \frac{1}{P(similar)}$ and that  of the `dissimilar' class is $w_0 = \frac{1}{1-P(similar)}$, where $P(similar)$ is the probability of two randomly selected documents being similar to each other.

Now, it is not possible to accurately compute P(similar), since all similar document-pairs cannot be known. Hence,
we devise two schemes to estimate the probability P(similar), Wtd-Sch 1 and Wtd-Sch 2, as described below.

\vspace{2mm}
\noindent \textbf{(i) Wtd-Sch 1}: In this scheme, the class weights are derived based on the hypothesis that if a document cites another document, they are likely to be similar (this hypothesis was previously applied in training data generation, as described in Section~\ref{ss:text-mtds-trng-data-gen}). 
The probability of the `similar' class is therefore the citation probability between two documents.

Consider the total number of case documents in our collection as $n_d$. Hence, there are ${n_d \choose 2}$ document-pairs in total. Consider that citation links exists between $n_c$ document pairs, i.e., $n_c$ document-pairs are similar according to the hypothesis stated above. Therefore, the probability of two documents being similar, P(similar) = $\frac{n_c}{{n_d \choose 2}}$.
In our corpus, $n_d = 53,211$, $n_c = 100,287$. Therefore, $P(similar)$ = $7.084 \times 10^{-5}$ and $1-P(similar)$ = $0.999$. Hence, $w_1$ = $14116.272$ and $w_0$ = $1.00007$.

\vspace{2mm}
\noindent \textbf{(ii) Wtd-Sch 2}: In this scheme, the class weights are derived based on the textual similarity between the case documents in the collection. We obtain the textual embeddings of the case documents from the trained Doc2Vec model (Section~\ref{ss:text-mtds-desc}). 
If  the cosine similarity between the Doc2Vec embeddings of the two documents is higher than $0.5$, we consider the document-pair to be `similar', else we consider the document-pair to be `dissimilar'. 
If there are ${n_d \choose 2}$ = $t$ document-pairs in the collection and among them $t_p$ are similar, then P(similar) = $\frac{t_p}{t}$.
Since it is computationally expensive to calculate ${n_d \choose 2}$ ($n_d$ = 53,211) similarity values, we calculate the weights based on 300 randomly sampled Civil cases and 300 randomly sampled Criminal cases. 
As these two types of cases are completely disjoint (refer to Section~\ref{ss:text-mtds-trng-data-gen}), we calculate the text similarity between these two sets of document-pairs separately.
Let $t_v$ be the number of Civil case document-pairs = $300 \choose 2$ = 44,850; similarly $t_r$ = number of Criminal case document-pairs= 44,850. 
We observe that $t_{p_{v}}$ = number of textually similar Civil case document-pairs is $6,387$ (based on the Doc2vec embeddings, as stated above) and $t_{p_{r}}$ is the number of textually similar Criminal case document-pairs is computed to be $12,662$. Therefore, we have $t$ = $t_v + t_r$ = $89,700$ and $t_p$ = $t_{p_{v}} +t_{p_{r}}$ = $19,049$. 
Hence, P(similar) =  $\frac{t_p}{t}$ = 0.212, $w_1$ = 4.708 and $w_0$ = 1.269.

\vspace{2mm}
\noindent Thus, in Wtd-Sch 1, the class weights are: $w_0$ = 1.00007, $w_1$ = 14116.272 and in Wtd-Sch 2, the class weights are: $w_0$ = 1.269,	$w_1$ = 4.708.


\begin{table}[t]
\caption{\new{Performance based on the weighted evaluation metrics of the different legal case document similarity methods, on the evaluation set. The best value is in \textbf{bold} ; second best value is \underline{underlined}. The "Unwtd." columns are repeated from earlier sections, for ease of reference.}}
\resizebox{\columnwidth}{!}{
\label{tab:eval-second}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Function}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{FScore}} & \multicolumn{3}{c|}{\textbf{MSE}} \\ \cline{4-9} 
 &  &  & \textbf{Unwtd.} & \textbf{Wtd-Sch 1} & \textbf{Wtd-Sch 2} & \textbf{Unwtd.} & \textbf{Wtd-Sch 1} & \textbf{Wtd-Sch 2} \\ \hline
% Text based &  & Doc2Vec & 0.774 & 0.738 & 0.753 & 0.0381 & 0.0414 & 0.0400 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Text\\ based \end{tabular}} & Unsupervised & Doc2Vec & 0.774 & 0.738 & 0.753 & \underline{0.0381} & 0.0414 & 0.0400 \\ \cline{2-9}
& Supervised & Concept Graph (Prec) & 0.694 & 0.758 & 0.739 & 0.1491 & 0.0554 & 0.0882 \\ \hline \hline
Network based &  & Hier-SPCNet-icf-m2v & 0.779 & 0.771 & 0.774 & 0.0427 & 0.0366 & 0.0393 \\ \hline \hline
% \multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Text\\ +\\ Network\\ \\ Combination\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Value\\ Combination\end{tabular}} & Val-avg & 0.828 & 0.817 & 0.822 & 0.039 & 0.0343 &  \\ \cline{3-9} 
% \multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Text\\ +\\ Network\\ \\ Combination\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Value\\ Combination\end{tabular}} & Val-avg & 0.828 & 0.817 & 0.822 & 0.039 & 0.0343 &  \\ \cline{3-9} 
%  &  & Val-max & 0.788 & 0.792 & 0.791 & 0.0375 & 2.72E-06 & 0.0081 \\ \cline{2-9} 
%  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Embedding\\ Combination\end{tabular}} & Emb-avg & 0.803 & 0.787 & 0.792 & 0.0382 & 2.67E-06 & 0.008 \\ \cline{3-9} 
%  &  & Emb-max & 0.705 & 0.773 & 0.75 & 0.0612 & 4.44E-06 & 0.0133 \\ \cline{3-9} 
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Text\\ +\\ Network \\ Combination\end{tabular}} & Value & Value-avg & 0.828 & \underline{0.817} & \underline{0.822} & 0.039 & 0.0343 & \underline{0.0351} \\ \cline{2-9} 
 & Embedding & Emb-Conc & \underline{0.829} & \underline{0.817} & \underline{0.822} & 0.0386 & 0.0355 &  0.0369\\ \cline{2-9} 
 & \multirow{2}{*}{Graph based} & Paper2Vec & 0.745 & 0.778 & 0.764 & 0.0598 & \underline{0.0225} & 0.0385 \\ \cline{3-9} 
 &  & TADW & 0.705 & 0.641 & 0.668 & 0.0619 & 0.0854 &  0.0753\\ %\cline{3-9} 
 \cline{2-9}
% &  & GCN & 0.385 & 0.662 & 0.544 & 0.2483 & 0.0633 &  0.1428 \\ \cline{3-9} 
 %&  & GraphSage & 0.678 & 0.761 & 0.726 & 0.1611 & 0.0720 & 0.1103 \\ \cline{2-9} 
 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Neural\\ Network\end{tabular}} & NN-Map+Conc & \textbf{0.829} & \textbf{0.828} & \textbf{0.829} & \textbf{0.0332} & \textbf{0.0183} & \textbf{0.0248} \\ \cline{3-9} 
 &  & NN-Map+Wtd Conc & 0.715 & 0.649 & 0.677 & 0.0424 & 0.0538 & 0.0489 \\ \cline{3-9} 
 \hline
 %&  & AE & 0.328 & 0.657 & 0.518 & 0.2558 & 0.0441 & 0.1351 \\ \hline
\end{tabular}
}
\end{table}


\new{\subsection{Results using weighted evaluation metrics}} 

Table~\ref{tab:eval-second} shows the performance of the different methods using the weighted metrics described above. 
We report values for the best and second best methods from each family of approaches. 
For each of the measures FScore and MSE, there are three columns -- Unwtd. where the values are repeated from  Table~\ref{tab:main-results}, Wtd-Sch 1 where FScore and MSE are weighted with class weights $w_0$ = 1.00007, $w_1$ = 14116.272, and Wtd-Sch 2 where they are weighed with class weights $w_0$ = 1.269, $w_1$ = 4.708. 

We find that all the metrics show NN-Map+Conc to be the best method. 
The Value-avg and Emb-Conc methods are second best performing methods in terms of weighted FScore. In terms of weighted MSE, Paper2Vec shows better result in Wtd-Sch 1 and Value-avg is better in Wtd-Sch 2. 
It can be noted that, for some methods like ConceptGraph and NN-Map+Wtd Conc, there is a notable difference between the unweighted (Unwtd.) metric values and the weighted metric values. 
This difference is because the methods are performing better for any one of the classes and worse for the other class. 
But our proposed methods Hier-SPCNet-icf-m2v (network-based) and NN-Map+Conc (text and network combined) have a balanced performance considering both unweighted and weighted metrics, thereby showing that they perform equally for both the similar and dissimilar document-pairs.

==> sections/problem.tex <==



The task/problem considered in this work is that of \textit{similarity estimation between two legal documents}. 
The input for this task is a pair of documents (which we term as a document-pair). 
The expected output is a \textit{single score} that reflects the level of similarity between the input document-pair.
Specifically, in this work, we consider the similarity score to be in the range $[0.0-1.0]$ where $0.0$ implies that the document-pair is least similar and $1.0$ implies that the two input documents are completely similar. 
The task of estimating document similarity is especially challenging in the legal domain, since legal documents are long, complicated and unstructured. 
Additionally, it is difficult to get large labelled datasets for training supervised Machine Learning/Deep Learning models for this task, since annotations by legal experts are very expensive.


%Note that, the similarity estimation problem is very different from a \textit{retrieval problem}, where the input is a \textit{single document} (query) and \new{documents \textit{that have already been cited} need to be ranked from a pool or repository of documents. }

A method for similarity estimation between a pair of documents can serve as a core internal module in applications like prior-case retrieval, recommendation, and so on.
In fact, we show the applicability of our proposed similarity estimation technique in recommending / retrieving uncited case documents for a source/query document, in Section~\ref{sec:reco-study}.

Nevertheless, the similarity estimation problem we consider in this work is quite different from a legal retrieval problem (where the input is a single query document and the intended output is a ranked list of `similar' documents).
As a result, the algorithms for similarity estimation (that we develop in this work) have to be evaluated differently from the common retrieval evaluation setup.
Specifically, we evaluate the algorithms for estimating similarity between two documents as follows.
For a particular input document-pair, an algorithm generates a similarity score in [0.0-1.0].
This algorithmically generated score is then evaluated against an expert-assigned similarity score for the same document-pair in the same range [0.0-1.0]. 
Based on these two scores (one from an algorithm and another from domain experts), both in the range [0.0-1.0], the algorithm is then evaluated using measures such as Pearson Correlation and Mean Squared Error (elaborated subsequently in Section~\ref{sub:evaluation-metrics}).


It can also be noted that, while there are several benchmark datasets available for evaluating legal retrieval algorithms (e.g.,~\cite{coliee-19}), to our knowledge, there are very few datasets available for evaluating algorithms for estimating the similarity between documents.
Hence, in this work, we develop a new dataset as described in the next section.




==> sections/results-text.tex <==
% \label{ss:results-text}

% \begin{table}[t]
% \centering
% \caption{Results of the different text and network based methods for computing  legal case document similarity. The best performing method is in \textbf{bold} ; second best performing method is \underline{underlined}.}
% \label{tab:text-results}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ Negative Examples\end{tabular}} & \textbf{Correlation} & \textbf{MSE} & \textbf{FScore} \\ \hline
%  \multirow{3}{*}{SMASH-RNN} & Random & 0.108 & 0.1085 & 0.557 \\ \cline{2-5}
% & Prec & 0.183 & \underline{0.1028} &  0.581\\ \cline{2-5} 
%  &  Prec+Text & 0.169 & 0.1622 & 0.542  \\ \hline
%  \multirow{3}{*}{SMASH-BERT} & Random & 0.209 & 0.2249 & 0.623\\ \cline{2-5}
%  & Prec & 0.255 & 0.1938 & 0.616  \\ \cline{2-5} 
%  &  Prec+Text & 0.232 & 0.2018 & 0.609 \\ \hline
%  \multirow{3}{*}{ConceptGraph} &  Random & 0.485 & 0.1751 & 0.610 \\ \cline{2-5}
%  & Prec & \underline{0.576} & 0.1491 & \underline{0.694} \\ \cline{2-5} 
%  &  Prec+Text &  0.551 & 0.1521 & 0.653 \\ \hline \hline
%  Doc2Vec & -- & \textbf{0.756} & \textbf{0.0452} & \textbf{0.793} \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\caption{Results of the text-based method (Doc2Vec) and best performing network-based method (Hier-SPCNet-ICF-m2v; values repeated from Table~\ref{tab:m2v-icfm2v}) for computing  legal case document similarity.}
\label{tab:text-results}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Type} & \textbf{Correlation} & \textbf{MSE} & \textbf{F-score} \\ \hline
 
 Doc2Vec & Text-based & 0.777 & 0.0381 & 0.774  \\ \hline
 Hier-SPCNet-ICF-m2v & Network-based & 0.725 & 0.0427 & 0.779  \\ \hline
 
\end{tabular}
\vspace{-6mm}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Negative sample\\ generation method\end{tabular}}} & \multicolumn{3}{c|}{\textbf{FScore}} & \multicolumn{3}{c|}{\textbf{MSE}} \\ \cline{3-8} 
%  &  & \textbf{Unwtd.} & \textbf{Wtd-Sch 1} & \textbf{Wtd-Sch 2} & \textbf{Unwtd.} & \textbf{Wtd-Sch 1} & \textbf{Wtd-Sch 2} \\ \hline
% \multirow{3}{*}{SMASH RNN} & Random & 0.557 & 0.422 & 0.477 & 0.1085 & 6.99E-06 & 0.0209 \\ \cline{2-8} 
%  & Prec & 0.581 & 0.529 & 0.551 & 0.1028 & 6.56E-06 & 0.0196 \\ \cline{2-8} 
%  & Prec+Text & 0.542 & 0.45 & 0.489 & 0.1622 & 6.77E-06 & 0.0203 \\ \hline
% \multirow{3}{*}{SMASH-BERT} & Random & 0.623 & 0.574 & 0.595 & 0.2249 & 0.0662 & 0.1048 \\ \cline{2-8} 
%  & Prec & 0.616 & 0.608 & 0.595 & 0.1938 & 1.30E-05 & 0.0391 \\ \cline{2-8} 
%  & Prec+Text & 0.609 & 0.621 & 0.616 & 0.2018 & 1.31E-05 & 0.0392 \\ \hline
% \multirow{3}{*}{ConceptGraph} & Random & 0.61 & 0.711 & 0.685 & 0.1751 & 0.0365 & 0.0390  \\ \cline{2-8} 
%  & Prec & 0.694 & 0.758 & 0.739 & 0.1491 & 0.0554 & 0.0882   \\ \cline{2-8} 
%  & Prec+Text & 0.653 & 0.724 & 0.701 & 0.1521 &  0.0615 & 0.0912 \\ \hline
% Doc2Vec (unsupervised) & -- & 0.774 & 0.738 & 0.753 & 0.0381 & 0.0414 & 0.0400  \\ \hline
% \end{tabular}
% \end{table}
We apply all the text-based methods described above (supervised and unsupervised) on the evaluation set of 100 document-pairs for which we have gold standard similarity scores from experts. We then measure Pearson Correlation, MSE, and F-score for each method,  which are stated in Table~\ref{tab:text-results}. 
%We find that the unsupervised method Doc2Vec performs the best across all the three evaluation metrics. Among the supervised methods, ConceptGraph performs best in terms of Correlation and FScore and SMASH-RNN in terms of MSE (both with the Prec strategy of generating negative examples). 




